Learning SQL from within: integrating database exercises into the database itself

SQL adventure builder (SQLab) is an open-source framework for creating SQL games that are embedded within the very database they query. Students' answers are evaluated using query fingerprinting, a novel technique that allows for better feedback than traditional SQL online judge systems. Fingerprints act as tokens that are used to unlock messages encrypted in an isolated auxiliary table. These messages may include hints, answer keys, examples, explanations, or narrative elements. They can also contain the problem statement of the next task, which turns them into nodes in a virtual DAG with queries as edges. This makes it possible to design a coherent adventure with a storyline of arbitrary complexity. This paper describes the theoretical underpinnings of SQLab's query fingerprinting model, its implementation challenges, and its potential to improve SQL education through game-based learning. The underlying concepts are fully cross-vendor, and support for SQLite, PostgreSQL and MySQL is already available. As a proof of concept, two games, 30 exercises and one mock exam were tested over a three-year period with about 300 students.

==> floats/same_result_queries_agg.tex <==

    \small\sffamily
    \begin{tabular}{l|cc|l}
    id. & $t_1$ & $t_2$ & raw query (before the injection of Formula~\ref{eqn:formulas:agg}) \\
    \hline
    $G_{1}$ & 1 &  & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(DISTINCT A.emp_id) FROM dependent A| \\
$G_{2}$ & 1 &  & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(*) FROM (SELECT emp_id, sum(hash) as hash FROM dependent GROUP BY emp_id) A| \\
$G_{3}$ & 3 &  & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(*) FROM employee A WHERE emp_id IN (SELECT emp_id FROM dependent)| \\
$G_{4}$ & 3 &  & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(*) FROM employee A WHERE EXISTS (SELECT 1 FROM dependent B WHERE A.emp_id = B.emp_id)| \\
$G_{5}$ & 5 &  & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT sum(EXISTS (SELECT 1 FROM dependent B WHERE A.emp_id = B.emp_id)) FROM employee A| \\
\hline
$O_{1}$ & 7 & 2 & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(DISTINCT A.emp_id) FROM dependent A JOIN dependent B ON A.emp_id = B.emp_id| \\
\cline{1-3}
$O_{2}$ & \textcolor{ACMOrange}{1} & 4 & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(DISTINCT A.emp_id) FROM dependent A JOIN employee B ON A.emp_id = B.emp_id| \\
$O_{3}$ & 9 & 4 & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(DISTINCT A.emp_id) FROM dependent B JOIN employee A ON A.emp_id = B.emp_id| \\
\hline
$I_{1}$ &  &  & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT 3 | \\
$I_{2}$ & \textcolor{ACMRed}{3} &  & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(*) FROM employee A WHERE emp_id IN ('123456789', '333445555', '987654321')| \\
\cline{1-3}
$I_{3}$ & \textcolor{ACMRed}{1} &  & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(DISTINCT relationship) from dependent A| \\
$I_{4}$ & \textcolor{ACMRed}{3} & 6 & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(*) FROM employee A JOIN dependent B ON A.emp_id = B.emp_id WHERE B.sex = 'M'| \\
$I_{5}$ & 11 & 6 & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(*) FROM employee B JOIN dependent A ON A.emp_id = B.emp_id WHERE A.sex = 'M'| \\
$I_{6}$ & 13 &  & \lstinline[basicstyle=\scriptsize\ttfamily,keepspaces=true]|SELECT count(*) FROM employee A WHERE salary = 25000| \\
    \end{tabular}
    
